Automated Deep Learning: Neural Architecture Search Is Not the End

Deep learning (DL) has proven to be a highly effective approach for developing models in diverse contexts, including visual perception, speech recognition, and machine translation. However, the end-to-end process for applying DL is not trivial. It requires grappling with problem formulation and context understanding, data engineering, model development, deployment, continuous monitoring and maintenance, and so on. Moreover, each of these steps typically relies heavily on humans, in terms of both knowledge and interactions, which impedes the further advancement and democratization of DL. Consequently, in response to these issues, a new field has emerged over the last few years: automated deep learning (AutoDL). This endeavor seeks to minimize the need for human involvement and is best known for its achievements in neural architecture search (NAS), a topic that has been the focus of several surveys. That stated, NAS is not the be-all and end-all of AutoDL. Accordingly, this review adopts an overarching perspective, examining research efforts into automation across the entirety of an archetypal DL workflow. In so doing, this work also proposes a comprehensive set of ten criteria by which to assess existing work in both individual publications and broader research areas. These criteria are: novelty, solution quality, efficiency, stability, interpretability, reproducibility, engineering quality, scalability, generalizability, and eco-friendliness. Thus, ultimately, this review provides an evaluative overview of AutoDL in the early 2020s, identifying where future opportunities for progress may exist.

==> IEEE_style/math_commands.tex <==
\usepackage{amsmath,amsfonts,bm}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}


% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}

% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sY{{\mathbb{Y}}}
\def\sD{{\mathbb{D}}}
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sR{{\mathbb{R}}}
\def\sK{{\mathbb{K}}}
\def\sT{{\mathbb{T}}}
\def\sI{{\mathbb{I}}}

\def\Figref#1{Figure~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\Algref#1{Alg.~\ref{#1}}
\def\Tabref#1{Table~\ref{#1}}
\def\Eqref#1{Eq.~\eqref{#1}}

==> fntml_style/MAL-editorialboard.tex <==
\begin{editorialboard}

\subsection{Editor-in-Chief}

\journalchiefeditor{Michael Jordan}{University of California, Berkeley\\United States}



\subsection{Editors}
\begin{multicols*}{3}\raggedcolumns
\journaleditor{Peter Bartlett}{UC Berkeley}
\journaleditor{Yoshua Bengio}{Universit{\'e} de Montr{\'e}al}
\journaleditor{Avrim Blum}{Toyota Technological Institute}
\journaleditor{Craig Boutilier}{University of Toronto}
\journaleditor{Stephen Boyd}{Stanford University}
\journaleditor{Carla Brodley}{Northeastern University}
\journaleditor{Inderjit Dhillon}{Texas at Austin}
\journaleditor{Jerome Friedman}{Stanford University}
\journaleditor{Kenji Fukumizu}{ISM}
\journaleditor{Zoubin Ghahramani}{Cambridge University}
\journaleditor{David Heckerman}{Amazon}
\journaleditor{Tom Heskes}{Radboud University}
\journaleditor{Geoffrey Hinton}{University of Toronto}
\journaleditor{Aapo Hyvarinen}{Helsinki IIT}
\journaleditor{Leslie Pack Kaelbling}{MIT}
\journaleditor{Michael Kearns}{UPenn}
\journaleditor{Daphne Koller}{Stanford University}
\journaleditor{John Lafferty}{Yale}
\journaleditor{Michael Littman}{Brown University}
\journaleditor{Gabor Lugosi}{Pompeu Fabra}
\journaleditor{David Madigan}{Columbia University}
\journaleditor{Pascal Massart}{Universit{\'e} de Paris-Sud}
\journaleditor{Andrew McCallum}{University of Massachusetts Amherst}
\journaleditor{Marina Meila}{University of Washington}
\journaleditor{Andrew Moore}{CMU}
\journaleditor{John Platt}{Microsoft Research}
\journaleditor{Luc de Raedt}{KU Leuven}
\journaleditor{Christian Robert}{Paris-Dauphine}
\journaleditor{Sunita Sarawagi}{IIT Bombay}
\journaleditor{Robert Schapire}{Microsoft Research}
\journaleditor{Bernhard Schoelkopf}{Max Planck Institute}
\journaleditor{Richard Sutton}{University of Alberta}
\journaleditor{Larry Wasserman}{CMU}
\journaleditor{Bin Yu}{UC Berkeley}
\end{multicols*}
\end{editorialboard} 

==> fntml_style/MAL-journaldata.tex <==
 \definecolor{palatinapurple}{rgb}{0.41, 0.16, 0.38}
\colorlet{MALcolor}{palatinapurple}   %new color names can be defined before use
\journalcolor      {MALcolor} %a color name.
\journaltitle      {Foundations and Trends\textsuperscript{\textregistered} in Machine Learning}
\journaltitleprefix{Foundations and Trends\textsuperscript{\textregistered} in}
\journalshorttitle {MAL}
\journalurl        {http://www.nowpublishers.com/MAL}
\journalissnprint  {1935-8237}
\journalissnonline {1935-8245}
\journaldoi        {10.1561/22}

\journalcopyrightowner{now Publishers Inc.}

\journalbibstyle{author} % either author or numeric

\journalaimsandscope
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
Machine Learning publishes
 survey and tutorial articles in the following topics:
 \begin{multicols}{2}\raggedcolumns
 \begin{itemize}
\item{Adaptive control and signal processing}
\item{Applications and case studies}
\item{Behavioral, cognitive and neural learning}
\item{Bayesian learning}
\item{Classification and prediction}
\item{Clustering}
\item{Data mining}
\item{Dimensionality reduction}
\item{Evaluation}
\item{Game theoretic learning}
\item{Graphical models}
\item{Independent component analysis}
\item{Inductive logic programming}
\item{Kernel methods}
\item{Markov chain Monte Carlo}
\item{Model choice}
\item{Nonparametric methods}
\item{Online learning}
\item{Optimization}
\item{Reinforcement learning}
\item{Relational learning}
\item{Robustness}
\item{Spectral methods}
\item{Statistical learning theory}
\item{Variational inference}
\item{Visualization}
\end{itemize}
\end{multicols}
 }


\journallibraryinfo
 {%
  Foundations and Trends\textsuperscript{\textregistered} in
  Machine Learning, \useissuedata{pubyear},
  Volume~\useissuedata{volume}, 6 issues.
  ISSN paper version \usejournaldata{issnprint}.
  ISSN online version \usejournaldata{issnonline}.
  Also available as a combined paper and online
  subscription.
 } 

==> fntml_style/MAL-seriespage.tex <==
\vspace{12pt}
\noindent \textit{Graph Kernels: State-of-the-Art and Future Challenges}\\
Karsten Borgwardt, Elisabetta Ghisu, Felipe Llinares-López, Leslie O’Bray and Bastian Rieck\\
ISBN: 978-1-68083-770-4\\
\\
\noindent \textit{Data Analytics on Graphs Part III: Machine Learning on Graphs, from Graph Topology to Applications}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-16\\
\\
\noindent \textit{Data Analytics on Graphs Part II: Signals on Graphso}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\
\\
\noindent \textit{Data Analytics on Graphs Part I: Graphs and Spectra on Graphs}\\
Ljubiša Stanković, Danilo Mandic, Miloš Daković, Miloš Brajović, Bruno Scalzo, Shengxi Li and Anthony G. Constantinides\\
ISBN: 978-1-68083-982-1\\

==> fntml_style/NOWFnT-data.tex <==
\newcommand\nowfnt@publicationaddress
 {%
  \textit{Published, sold and distributed by:}\\
  now Publishers Inc.\\
  PO Box 1024\\
  Hanover, MA 02339\\
  United States\\
  Tel.\ +1-781-985-4510\\
  www.nowpublishers.com\\
  sales@nowpublishers.com%
  \par
  \textit{Outside North America:}\\
  now Publishers Inc.\\
  PO Box 179\\
  2600 AD Delft\\
  The Netherlands\\
  Tel.\ +31-6-51115274
 }

\newcommand\nowfnt@legalrightstext
 {%
  All rights reserved. No part of this publication may be
  reproduced, stored in a retrieval system, or transmitted in any form or by any means, mechanical, photocopying, recording or otherwise, without prior written permission of the publishers.
  \par
  Photocopying. In the USA: This journal is registered at the Copyright  Clearance Center, Inc., 222 Rosewood Drive, Danvers, MA 01923.  Authorization to photocopy items for
  internal or personal use, or the internal or personal use of specific  clients, is granted by now Publishers Inc for users registered with the Copyright Clearance Center (CCC).
  The `services' for users can be found on the internet at:
  www.copyright.com
  \par
  For those organizations that have been granted a photocopy license, a separate system of payment has been arranged. Authorization does not extend to other kinds of copying, such as that for general distribution, for advertising or promotional purposes, for creating new collective works, or for resale.  In the rest of the world:
  Permission to photocopy must be obtained from the copyright
  owner. Please apply to now Publishers Inc., PO Box 1024, Hanover, MA 02339, USA; Tel. +1 781 871 0245; www.nowpublishers.com; sales@nowpublishers.com
  \par
  now Publishers Inc. has an exclusive license to publish this
  material worldwide. Permission to use this content must be obtained from the copyright license holder. Please apply to now Publishers, PO Box 179, 2600
  AD Delft, The Netherlands, www.nowpublishers.com; e-mail:
  sales@nowpublishers.com}

\newcommand\nowfnt@printedoninfotext
 {%
  {%
   %
  }%
 }

\newcommand\nowfnt@howtocitetext
 {%
  The preferred citation for this publication is\par
  {%
   \raggedright
   \useissuedata{copyrightowner}.
   \emph{\nowfnt@articletitle}.
   \printjournaltitleprefix \usejournaldata{title}, vol.~\useissuedata{volume}, no.~\useissuedata{issue}, pp.~\useissuedata{firstpage}--\useissuedata{lastpage},
   \useissuedata{pubyear}.%
  }%
 }


\newcommand\nowfnt@copyrightlinetext
 {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} \useissuedata{copyrightowner}}

\newcommand\nowfnt@NOWcopyrightlinetext  %for wrapper
  {%
  ISBN: \useissuedata{isbn}\\
  \copyright\ \useissuedata{copyrightyear} Now Publishers Inc}

\newcommand\nowfnt@sourceintro{%
 The content of the book was originally published in  }

\newcommand\nowfnt@sourcepunct{.}

\newcommand\nowfnt@prohibitiontext{This article may be used only for the purpose of research, teaching, and/or private study. Commercial use or systematic downloading (by robots or other automatic processes) is prohibited without explicit Publisher approval.}

\newcommand\nowfntstandardcitation{\nowfnt@authorlist@toc\ (\nowfnt@issuepubyear), \enquote{\nowfnt@articletitle}, \nowfnt@journaltitle: Vol. \nowfnt@issuevolume, No. \nowfnt@issueissue, pp \nowfnt@issuefirstpage--\nowfnt@issuelastpage. DOI: \nowfnt@issuedoi.}

%Title for the series pages.
\newcommand\nowfnt@seriespagetitle{\section*{Other titles in \nowfnt@journaltitle}}

==> fntml_style/math_commands.tex <==
\usepackage{amsmath,amsfonts,bm}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}


% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}

% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sY{{\mathbb{Y}}}
\def\sD{{\mathbb{D}}}
\def\sE{{\mathbb{E}}}
\def\sF{{\mathbb{F}}}
\def\sR{{\mathbb{R}}}
\def\sK{{\mathbb{K}}}
\def\sT{{\mathbb{T}}}
\def\sI{{\mathbb{I}}}

\def\Figref#1{Figure~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\Algref#1{Alg.~\ref{#1}}
\def\Tabref#1{Table~\ref{#1}}
\def\Eqref#1{Eq.~\eqref{#1}}

==> tables/table-ade.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
Evaluative assessment for trends in automated data engineering.
}
    \begin{tabular}{l | l | l | l | l | l | l | l | l | l | l | l}
    \toprule
 &                   & Novelty           & Solution & Effic. & Stability & Interp. & Reprod.  & Engi. & Scalability   & General. & Eco. \\
\midrule
% \multirow{2}{*}{\rotatebox[origin=c]{90}{\makecell{Make\\more\\data}}}
\multirow{2}{*}{\makecell[l]{Supplementary\\Generation}}
 & data generation   & $\approx$ 2 (30) & Low   &   Low     & Low     & High          & ?  & ?     & ?    & Low    & ?  \\\cmidrule{2-12}
 & label generation  & $\approx$ 2 (40) & High  &   Low     & High    & Low           & ?  & ?     & High   & Low    & ?  \\
\midrule
\multirow{2}{*}{\makecell[l]{ Intelligent\\Exploitation}}
 & data augmentation & $\approx$ 5 (30) & High  &   Mixed   & High    & Low           & ?  & ?     & High   & Low    & ?  \\\cmidrule{2-12}
 & data selection    & $\approx$ 4 (30) & Medium  &  Mixed     & High    & High       & ?  & ?     & High    & High   & ?  \\
    \bottomrule
    \end{tabular}
    \label{table:ade-methods}
    \end{center}
    \textit{
    Each row marks an emergent trend in AutoDL, specifically automated data engineering. Each column marks a criterion -- see \Secref{sec:criteria-intro} -- by which the trend is assessed. The evaluations are mostly qualitative, averaged across the most significant works researching the trend. Where a graded value is not provided, ``?'' indicates that a rigorous assessment is not achievable without more research works to analyze.  Novelty denotes years since seminal works in DL (ML) were published. Abbreviations are: ``Solution'' for Solution Quality, ``Effic.'' for Efficiency, ``Interp.'' for Interpretability, ``Reprod.'' for Reproducibility, ``Engi.'' for Engineering Quality, ``General.'' for Generalizability, and ``Eco.'' for Eco-friendliness. 
    % Each column is a relative evaluation between the two sub-areas.
    % This evaluation is for the majority of works in that area instead of a specific work/paper.
    % ``?'' indicates that it is unclear due to the lack of strong evidence or the need for more investigation.
    % ``Effic.'' and ``Interp.''  indicate ``Efficiency'' and ``Interpretability''.
    % ``Reprod.'', ``Engi.'', and ``Gene.'' are ``Reproducibility'', ``Engineering quality'', and ``generalizability'', respectively.
    }
    % Majority vs. Minority
    % Overarching assessment
    % More precise years: approximately xxx years
    % 
    % Accuracy:
    %   -- data generation: too novel and only experiment on small datasets. In some offline discuss, the authors said it does not work at the momentum.
    %   -- label generation: self-training-based solutions have been studied for many years. Even if without auto-dl, heuristic strategy is already good and augmenting it with Auto-DL becomes better.
    %   -- data augmentation: augmentation is a very strong technique to augment the performance. Based on the existing augmentation solutions, auto data augmentation can boost the performance compared to baseline augmentation by a large margin.
    %   -- data selection: currently auto-selection only experiment on small-scale datasets, and its upper bound is usually limited by using all data.
    % Efficiency:
    %   -- data generation: need to train generators and by generating more data, the cost becomes much larger.
    %   -- label generation: self-training-based paradigm usually needs to iteratively optimize the model and generate labels for unlabeled data, and re-optimize the model, re-generate, ...., One iteration's cost can be tens of GPU hours, not to mention that for many iterations.
    %   -- data augmentation: depends what search algorithms (weight-sharing-based or multi-trial-based) is used.
    %   -- data selection: if it is online batch-level selection, then the algorithm is usually efficient; if it is offline selection, then it may encounter the similar issue as that in `label generation`.
    % Stability: 
    %   -- data generation: the current status of research is still in experimental stage.
    %   -- label generation: absorbed from that in the broader ML domain, the auto-dl algorithm is stable. 
    %   -- data augmentation: in the paper and given my experience, the current algorithm is stable on vision problems. That on others may need more investigation.
    %   -- data selection: Given the numbers in papers, it is stable.
    % Interp.
    %   -- data generation, has some theoretical analysis, and generated data can be visualized for better analysis.
    %   -- label generation, that in Auto-DL does not have theoretical analysis yet.
    %   -- data augmentation, no much theoretical analysis
    %   -- data selection, gradient-based solutions has some math formulations with analysis on how to approximate the hyper-gradients.
    % Reprod.
    %   -- All of them are not been benchmarked yet in Auto-DL.
    % Engi.
    %   -- All of them does not have a good lib yet (given my impression).
    % Scalability.
    %   -- data generation, too early stage.
    %   -- label generation, the time is linearly scalable to the size of dataset.
    %   -- data augmentation, linearly scalable to the size of dataset.
    %   -- data selection, linearly scalable to the size of dataset.
    % Gene.
    %   -- data generation / label generation / data augmentation are usually task/application-specific, and thus lacks generalization ability
    %   -- data selection, the method can generalize to different tasks as it does not care about the data structure / format / formulation / etc.
\end{table*}

==> tables/table-dep.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
Evaluative assessment for trends in automated deployment.
}
\begin{tabular}{l | l | l | l | l | l | l | l | l | l | l}
    \toprule
                            & Novelty      & Solution & Effic. & Stability & Interp. & Reprod.  & Engi. & Scalability   & General. & Eco. \\
\midrule
    Deployment-aware AutoDL & $\approx$ 4  &   High   &  Mixed     & Medium    & High    & \cmark   &   ?    & Mixed         & Mixed            & Mixed  \\
    Hardware Search         & $\approx$ 5  &   High   &  Low       & ?         & Low     & ?        &   ?    & Low           & Low              & ?  \\
    \bottomrule
    \end{tabular}
    \label{table:dep-methods}
    \end{center}
    \textit{
    Each row marks an emergent trend in AutoDL, specifically automated deployment. Each column marks a criterion -- see \Secref{sec:criteria-intro} -- by which the trend is assessed. The evaluations are mostly qualitative, averaged across the most significant works researching the trend. Where a graded value is not provided, ``\cmark'' indicates a rigorous assessment is possible with analysis beyond the scope of this review, while ``?'' indicates that not even this is achievable without more research works to analyze. Novelty denotes years since seminal works in DL were published. Abbreviations are:  ``Solution'' for Solution Quality, ``Effic.'' for Efficiency, ``Interp.'' for Interpretability, ``Reprod.'' for Reproducibility, ``Engi.'' for Engineering Quality, ``General.'' for Generalizability, and ``Eco.'' for Eco-friendliness. 
    }
% Explaination:
% Accuracy: Both of them can achieve a high accuracy at the end of the pipeline.
% Efficiency: Deployment-aware AutoDL can be high (if using gray-box-based search algorithm) or low (if using white-box-based-search algorithm)
%             Hardware Search usually utilized gray-box-based search algorithm, and is thus low.
% Stability:
%         -- Deployment-aware AutoDL is somewhat stable given my experience but lacks systematical analysis
%         -- Hardware Search: only few works, most does not report Stability analysis, due to the expensive cost of hardware search other people are difficult to evaluate the stability.
% Interp.: TBD
% Reprod.: \cite{li2021hw} is the one for deployment-aware AutoDL
% Engi.: there are a few highly-GitHub-started repos for Deployment-aware AutoDL, but does not meet the detailed criteria we listed in the final table
% Scalability:
%         Deployment-aware AutoDL can be high (if using white-box-based-search algorithm) or low (if using gray-box-based search algorithm)
%         Hardware Search is low as it is too expensive
% Generalizability:
%         Deployment-aware AutoDL can be high (if using gray-box-based search algorithm) or low (if using white-box-based-search algorithm)
%         Hardware Search is usually task, hardware-type -specific
\end{table*}

==> tables/table-hpo.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
Evaluative assessment for trends in HPO.
}
\begin{tabular}{l | l | l | l | l | l | l | l | l | l | l}
    \toprule
                                  & Novelty & Solution & Effic. & Stability & Interp. & Reprod.  & Engi. & Scalability   & General. & Eco. \\
\midrule
    Black-box HPO & $\approx$ 30  & High    & Low    & High   & High         & \cmark    & \cmark  & Low  & High  & Low  \\
    Gray-box HPO  & $\approx$ 30  & Medium  & Medium & Medium & Medium       & \cmark    & \cmark  & Low  & High  & Medium  \\
    White-box HPO & $\approx$ 21  & Medium  & High   & Low    & Medium       & ?         & ?    & High & Low   & High  \\
    \bottomrule
    \end{tabular}
    \label{table:hpo-methods}
    \end{center}
    \textit{
    Each row marks an emergent trend in AutoDL, specifically HPO. Each column marks a criterion -- see \Secref{sec:criteria-intro} -- by which the trend is assessed. The evaluations are mostly qualitative, averaged across the most significant works researching the trend. Where a graded value is not provided, ``\cmark'' indicates a rigorous assessment is possible with analysis beyond the scope of this review, while ``?'' indicates that not even this is achievable without more research works to analyze. Novelty denotes years since seminal works in ML were published. Abbreviations are: ``Solution'' for Solution Quality, ``Effic.'' for Efficiency, ``Interp.'' for Interpretability, ``Reprod.'' for Reproducibility, ``Engi.'' for Engineering Quality, ``General.'' for Generalizability, and ``Eco.'' for Eco-friendliness. 
    }
% Novelty:
%   -- Black-box and gray-box: 
%   -- White-box: \cite{bengio2000gradient} 21 years.
% Accuracy & efficiency:
%   -- Black-box: The best performance as each candidate is fully optimize / computed, but the efficiency is the lowest.
%   -- Gray-box: trade-off the accuracy and efficiency compared to black-box
%   -- White-box: accuracy is relatively lower than black-box, while the efficiency is significantly boosted.
% Stability:
%   -- Black-box is more stable, while it depends on 
% Interp.
%   -- TBD
% Reprod.: has it been benchmarked and systemtically evaluated for benchmarking.
%   -- black-box and gray-box are usually implemented in a unified way, as black-box can be viewed as a special case of gray-box.
%   -- as for the white-box, I do not remember if there is any work on that.
% Engi.:
%   -- black-box and gray-box has good libraries due to the long history.
%   -- white-box is more domain/application/algorithm-specific, and I do not remember there is a good lib.
% Scalability:
%   -- Black-box and gray-box are less scalable as both of them requires costly train/evaluation for DL Models.
%   -- white-box is scalable as it is efficient.
% Generalizability:
%   -- Black-box and gray-box do not have much assumption and constraints for the application, search space, tasks, and are thus generalizable.
%   -- white-box: usually has many implicit or explicit assumptions that needs additional modification to generalize to other search spaces or applications.
\end{table*}

==> tables/table-maint.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
Evaluative assessment for trends in automated maintenance.
}
\begin{tabular}{l | l | l | l | l | l | l | l | l | l | l}
    \toprule
                        & Novelty         & Solution & Effic. & Stability & Interp. & Reprod.  & Engi. & Scalability & General. & Eco. \\
\midrule
    Domain Adaptation   & 3 ($\approx$30) & ?        &  High  &  ?        &    ?    &     ?    &   ?   &    High     &   Mixed  &   ?  \\
    Low-shot Learning   & 3 ($\approx$29) & ?        &  High  &  ?        &    ?    &     ?    &   ?   &    High     &   Mixed  &   ?  \\
    Continuous Learning & 5 ($\approx$30) & ?        &  High  &  ?        &    ?    &     ?    &   ?   &    High     &   Mixed  &   ?  \\
    % Auto-Concept Drift       & 2 ($\approx$33) & ? &  ?       &  ?  & ? &  ?  &  ? &  ?      &   ?     & ? \\
    % Deep RL             & 5               & ? & Mixed    &  ?  & ? &  ?  &  ? & Mixed   &  Medium   & ? \\
    \bottomrule
    \end{tabular}
    \label{table:maint-methods}
    \end{center}
    \textit{
    Each row marks an emergent trend in AutoDL, specifically automated maintenance. Each column marks a criterion -- see \Secref{sec:criteria-intro} -- by which the trend is assessed. The evaluations are mostly qualitative, averaged across the most significant works researching the trend. Where a graded value is not provided, ``?'' indicates that a rigorous assessment is not achievable without more research works to analyze.  Novelty denotes years since seminal works in DL (ML) were published. Abbreviations are: ``Solution'' for Solution Quality, ``Effic.'' for Efficiency, ``Interp.'' for Interpretability, ``Reprod.'' for Reproducibility, ``Engi.'' for Engineering Quality, ``General.'' for Generalizability, and ``Eco.'' for Eco-friendliness. 
    }
% Explainations:
% Novelty:
%     - domain adaptations : \cite{li2020adapting}
%     - low-shot learning  :  (\cite{larochelle2008zero,lake2011one,schein2002methods,schmidhuber1992learning})
%     - Continual Learning : 
%     - Concept Drift      : \cite{basseville1993detection}
% Accuracy: all is ?, because they target different applications, and it is impossible to compare
% Efficiency: most of AutoDL for Domain Adaptation, Low-shot Learning, Continual Learning are gradient-based, which are thus high efficient.
%     - In AutoRL, some works utilized black-box-based methods, which are inefficient due to the multi-trial nature; some are gradient-based, which are efficient 
% Stability:
%     AutoDL for Domain Adaptation, Low-shot Learning, Continual Learning have not been formally been identified as a research area, and not to mention some benchmark or stability analysis.
%.    AutoRL does not have benchmarks yet.
% Interp.: TBD
% Reprod.: there are too few works to consider the reproducibility issues for these four areas
% Engi.: does not have much good repos for AutoDL in these sub-domains
% Scalability:
%     sharing the similar reasons for "Efficiency". Gradient-based methods are efficient and thus can Scalabile to larger model / datasets. AutoRL is mixed as some are scalabile and some are not.
% Generalizability: we define generalizability as generalize to other search spaces.
%     For Domain Adaptation / Low-shot Learning / Continual Learning, it depands on the specific methods, some are specifically designed for the model head (such as the classification layer), or other componeats, and thus maynot be easily generalized to other search spaces.
%    - AutoRL: as RL has many components, some focused on automating the objective function and some focused on automating the architecture. These methods can not easily be used for a different search space.
\end{table*}

==> tables/table-nas.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
Evaluative assessment for trends in NAS.
}
    \begin{tabular}{l | l | l | l | l | l | l | l | l | l | l | l}
    \toprule
      &                       &   Novelty     & Solution & Effic. & Stability & Interp. & Reprod.  & Engi. & Scalability   & General. & Eco. \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell{Search\\Space}}}
      & Size-related          &  $\approx$20  & Medium   & Medium & High      & ?     & \cmark   &  \cmark  & High      &  High & ?  \\
      & Conv: NASNet-like     &  $\approx$4   & High     & Low    & Medium    & ?     & \cmark   &  ?  & Medium    &  High & ?  \\
      & Conv: MBConv-based    &  $\approx$3   & High     & Mixed  & High      & ?     & ?        &  \cmark  & High      &  High & ?  \\
      & Others                &  $\approx$10  & Mixed    & Mixed  & Mixed     & ?     & ?        &  ?  & Mixed     &  Low  & ?  \\
\midrule
\multirow{4}{*}{\rotatebox[origin=c]{90}{\makecell{Search\\Strategy}}}
      & RL-based              &  $\approx$5   & High        & Mixed    &  ?      & Medium  & \cmark    &  \cmark & High   & High & ?      \\
      & Evolutionary          &  $\approx$10  & High        & Mixed    &  ?      & Medium  & \cmark    &  \cmark & High   & High & Mixed      \\
      & BayesOpt-based        &  $\approx$9   & High        & Mixed    &  ?      & Medium  & \cmark    &  \cmark & Medium & High & ?      \\
      & Differentiable        &  $\approx$3   & Medium        & High   &  ?      & Medium  & \cmark    &  ?   & High   & High & ?      \\
\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{\makecell{Candidate\\Evaluation\\Boosts}}}
      &  Heuristic low-fidelity approx. & $\approx$10 &  High    & Low     & Mixed    & ?    & \cmark &  ?  &  Low    & High   & ?\\
      &  Neural predictor               & $\approx$6  &  Medium  & Low     & Mixed    & ?    & \cmark &  ?  &  Low    & High   & ?\\
      &  Weight generation/inheritance  & $\approx$6  &  Medium  & Medium  & Medium   & ?    & ? &  ?  &  Medium & Medium & ?\\
      &  Weight sharing                 & $\approx$3  &  Medium  & Medium  & Low      & ?    & ? &  ?  &  High   & Medium & ?\\
      &  NAS without training           & $\approx$1  &  Low     & High    & ?        & ?    & ? &  ?  &  Mixed  & ?      & ?\\
    \bottomrule
    \end{tabular}
\label{table:nas-methods}
\end{center}
    \textit{
    Each row marks an emergent trend in AutoDL, specifically NAS. Each column marks a criterion -- see \Secref{sec:criteria-intro} -- by which the trend is assessed. The evaluations are mostly qualitative, averaged across the most significant works researching the trend. Where a graded value is not provided, ``\cmark'' indicates a rigorous assessment is possible with analysis beyond the scope of this review, while ``?'' indicates that not even this is achievable without more research works to analyze. Novelty denotes years since seminal works in DL were published. Abbreviations are: ``Solution'' for Solution Quality, ``Effic.'' for Efficiency, ``Interp.'' for Interpretability, ``Reprod.'' for Reproducibility, ``Engi.'' for Engineering Quality, ``General.'' for Generalizability, and ``Eco.'' for Eco-friendliness. 
    }
%% Add BayesOpt-based NAS in Sec.5.2
%% Re-f Sec.5.1
% Explanations --- Search Space
% - Accuracy: NASNet-like and MBConv-based are both high, size-based are ok, in others, there are too many cases
% - Efficiency:  NASNet-like runs very slow, MBConv-based can be fast when using weight-sharing, while is slow when using multi-trial
% - Scalability: NASNet-like is usually harder to converge than MBConv / Size -based.
% - Interp.: there are no theoritcal analysis for search space.
% - Reprod.: MBConv-based or Size-related search spaces are relatively simpler than NASNet-like
% - Engi.:
%    -- NasNet-like space needs to be represented as a graph, and there is current no popular and easy-to-use lib for it.
%    -- MBConv-based or Size-related is simpler and can be represented by a list of choices -- like selecting hyperparameters in a sequential way. Many HPO or NAS libs can easily support that.
%    -- Others: too many variants and do not have a good lib can unify the codes.
% - Scalability
%    -- When the NASNet-like space increased, the search difficulty will be significantly increased, as the choices at each node and edges are strongly coupled.
%    -- When build candidate architecture in MBConv-based or Size-related, each choice is loosely coupled with another one. Such as, the configuration at one layer only has not much effect for the config at next layer.
%    -- Others: too many variants..
% - Gene.: Other search spaces are usually customized for specific applications (usually a downstream task), which is less transferrable to other applications.
%
% Explanations --- Search Strategy
% - Novelty: Bayesian-based NAS may start from \cite{bergstra2013making} and \cite{snoek2012practical}
% - Accuracy: no conclusion for which is better, in different papers, one can be better than others, but in a different paper, the conclusion can reverse. However, generally speaking, every algorithm can achieve good performance finally.
% - Eff: RL/Evolution/BayesOpt typically is multi-trial-based solution, which is slow. (although they can be fast when using weight sharing)/
% - Stability: only has little study in benchmark papers.
% - Interp.: all of them have theoritical analysis, but the conditions usually do not hold in practice, as many approximation or proxy are introduced. This can obscure
% - Reprod.: Depand on specific paper, some are reproduciable and some are not...
% - Engi.: RL/Evolution/BayesOpt have been studied for many years and thus have some good libraries, but RL/Evo/BayesOpt for NAS do not have as good lib as that in a broader area..
% - Scalability: BayesOpt is limited to the size of embedding of candidates, BayesOpt can maximumly handle hundresds of dims.
% - Gene.: all search algorithms are generally applicable to any application or search spaces.
%
% Explanations --- Evaluate Candidate
% - Accuracy: Heuristic low-fidelity approx. can best estimate the performance but cost most.
%     -- Neural predictor, Weight generation/inheritance, Weight sharing involves much approximations and is not that accurate as low-fidelity.
%     -- NAS without training, as no training is involved, the estimation of architecture ranking is less reliable.
% - Effic.: Heuristic low-fidelity approx and Neural Predictor need to train and evaluate some candidate architectures, which are expensive. Others do not need to do so.
% - Stability: Heuristic low-fidelity approx. and Predictor are mixed, as it depends which proxy task is used.
% - Interp. and Reprod. : to the best of my knowledge, it is not studied yet.
%     -- low-fidelity approx..: one work is \cite{eggensperger2021hpobench}
%     -- Neural predictor: \cite{NAS-Bench-x11}
% - Engi.: no good libs for these strategies.
% - Scalability: Heuristic low-fidelity approx. and Neural predictor are linear to the size of search space.
%                Weight generation/inheritance also need to explore more candidates as the search space grows.
%                Weight sharing can be views as a "log" relationship of the size of search space.
%                NAS without training needs to compute some metrics in unsupervised way. Its Scalability depends on how the metrics are computed.
% - Gene.:
%     -- Heuristic low-fidelity approx. and Neural predictor are usually agnostic to the architecture design and thus is more general.
%     -- Weight generation/inheritance and Weight sharing is customized according to specific architecture / search space.
%     -- NAS without training: need more deep dive for its generalization ability, currently only has little studies.
\end{table*}

==> tables/table-optim.tex <==
\begin{table*}[!htb]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
AutoDL algorithms dissected as optimization strategies.
}
\begin{tabular}{ c | l | l | l | l | l }
\toprule
            & Algorithm & Search Space & Search Strategy & Boosts for Candidate Evaluation & Application \\
\midrule
\multirow{10}{*}{\rotatebox[origin=c]{90}{Auto Data Engineering}}
      & \cite{maclaurin2015gradient} 2015.02 & training data                     & Differential  & optimal storage of discarded entropy & CLS: MNIST \\
    %   & \cite{konyushkova2017learning} 2017.03 & data selection &  \\
      & \cite{fan2018learning} 2018.05       & training data selection           & REINFORCE     & weight sharing; mini-batch sample    & CLS: MNIST/CIFAR/IMDB \\
      & \cite{ren2018learning} 2018.03       & training data re-weight           & Differential  & weight sharing; online approximation & CLS: MNIST/CIFAR \\
    %   & \cite{shu2019meta} 2019.02           & data weight      & Differential \\
      & \cite{cubuk2019autoaugment} 2018.05  & transformation in PIL~\cite{pil}  & PPO           & smaller model; reduced dataset & CLS: five datasets \\
      & \cite{lim2019fast} 2019.05           & transformation in PIL             & BayesOpt      & weight sharing                 & CLS: four datasets \\
      & \cite{zoph2020learning} 2019.06      & transformation in PIL             & PPO           & reduced dataset                & Object DET: VOC/COCO     \\
      & \cite{niu2019automatically} 2019.09  & classical NLP augmentations       & REINFORCE     & fewer epochs                   & Dialogue tasks       \\
      & \cite{cubuk2020randaugment} 2019.09  & transformation in PIL             & Random        & smaller model; reduced dataset & CLS + Object DET \\
      & \cite{such2020generative} 2019.12    & training data                     & Differential  & weight normalization           & CLS + Game: CartPole \\
      & \cite{li2020differentiable} 2020.03  & transformation in PIL             & Differential  & reduced dataset                & CLS + Object DET \\
\midrule
\multirow{27}{*}{\rotatebox[origin=c]{90}{Neural Architecture Search}}
      & \cite{bayer2009evolving} 2009.09         & cell topology in LSTM             & Evolution    &     N/A                                 & Grammar benchmarks      \\
      & \cite{jozefowicz2015empirical} 2015.07   & topology and operation in LSTM    & Evolution    & easy-to-hard tasks to filter            & Music + Language        \\
      &  \cite{zoph2017NAS} 2016.11              &  filter size + connectivity       & PPO          & fewer epochs                            & CLS + Language tasks    \\
      & \cite{baker2017designing} 2016.11        & MetaQNN space                     & Q-learning   & fewer epochs; early stop                & CLS: four datasets  \\
      & \cite{real2017large} 2017.03             & unrestricted CNN space            & Evolution    & weight inheritance                      & CLS: CIFAR-10/100   \\
      & \cite{zoph2018learning} 2017.07          & NASNet space                      & PPO          & fewer epochs                            & CLS + Object DET    \\
      & \cite{brock2018smash} 2017.08            & SMASH space                       & Random       & weight generation via HyperNet~\cite{ha2017hypernetworks} & CLS: five datasets \\
      & \cite{zhong2018practical} 2017.08        & BlockQNN space                    & Q-learning   & early stop                              & CLS: CIFAR/ImageNet    \\
      & \cite{ramachandran2017searching} 2017.10 & activation functions              & PPO          & smaller model                           & CLS + Translation      \\
      & \cite{real2019regularized} 2018.02       & NASNet space                      & Evolution    & smaller model; fewer epochs             & CLS: CIFAR/ImageNet    \\
      & \cite{pham2018efficient} 2018.02         & reduced NASNet space (RNS)        & REINFORCE    & weight sharing~\cite{pham2018efficient} & CLS + Language tasks \\
      & \cite{liu2019darts} 2018.06              & reduced NASNet space              & Differential & weight sharing; smaller model; etc      & CLS + Language tasks  \\
      & \cite{cai2018path} 2018.06               & tree-structure                    & REINFORCE    & Net2Net~\cite{chen2016net2net}          & CLS: CIFAR/ImageNet \\
      & \cite{tan2019mnasnet} 2018.07            & MBConv-based space (MBS)          & PPO          & fewer epochs                            & CLS + object DET       \\
      & \cite{bender2018understanding} 2018.07   & modified NASNet space             & Random       & weight sharing                          & CLS: CIFAR/ImageNet    \\
      & \cite{luo2018neural} 2018.08             & reduced NASNet space              & Differential & weight sharing; neural predictor        & CLS + language  \\
    %   & \cite{zhang2019graph} 2018.10            & reduced NASNet space              & Random       &  weight generation via HyperNet & image classification \\
      & \cite{cai2019proxylessnas} 2018.12       & MBConv-based space                & Differential & weight sharing                          & CLS: CIFAR/ImageNet  \\
      & \cite{liu2019auto} 2019.01               & RNS + connectivity                & Differential & weight sharing; smaller model           & SEG: three datasets  \\
    %   & \cite{li2020random} 2019.02              & reduced NASNet space              & Random       & weight sharing; smaller model & image classification \\
      & \cite{chen2019detnas} 2019.03            & ShuffleNetv2-based backbone       & Evolution    & weight sharing                          & CLS + object DET     \\
    %   & \cite{quan2019auto} 2019.03 & reduced NASNet space + part-aware op & differentiable & weight sharing; smaller model & person re-ID \\
      & \cite{xie2019exploring} 2019.04          & architecture generator space      & manual       & fewer epochs                            & CLS + object DET     \\
      & \cite{ghiasi2019fpn} 2019.04             & FPN space                         & PPO          & smaller model; fewer epochs             & object DET: COCO     \\
      & \cite{dong2019tas} 2019.05               & depth + width                     & Differential & weight sharing                          & CLS: CIFAR/ImageNet  \\
    %   & \cite{dong2019search} 2019.06 & reduced NASNet space & Differential & weight sharing; Gumbel & image classification \\
      & \cite{fang2020densely} 2019.06           & densely connected search space    & Differential & weight sharing                          & CLS + object DET \\
    %   & \cite{xu2020pc} 2019.07 & reduced NASNet space & Differential & weight sharing; partial connection & image classification \\
    %   & \cite{du2020spinenet} 2019.12            & scale-permuted space              &  PPO         & smaller model; fewer epochs & object detection \\
      & \cite{ru2020neural} 2020.04              & architecture generator space      & BayesOpt     & fewer epochs                            & CLS: six datasets \\
      & \cite{liu2020evolving} 2020.04           & normalization+activation          & Evolution    & smaller dataset; fewer epochs           & CLS + SEG + GAN \\
      & \cite{wan2020fbnetv2} 2020.04            & width + resolution                & Differential & weight sharing                          & CLS: ImageNet \\
    %   & \cite{dai2021fbnetv3} 2020.06            & MBS + HPs                         & Evolution    & predictor; fewer epochs & image classification \\
    %   & \cite{tang2021auto} 2021.01              & reduced NASNet space              & Differential & weight sharing & navigation \\
\midrule
\multirow{10}{*}{\rotatebox[origin=c]{90}{Hyperparameter Opt.}}
      & \cite{bengio2000gradient} 1999.09     & a few differentiable HPs       & Differential    & N/A                                              & Synthetic data \\
      & \cite{snoek2012practical} 2012.06     & a few HPs                      & BayesOpt        & modeling costs; parallel                         & Diverse tasks \\
      & \cite{maclaurin2015gradient} 2015.02  & hundreds of differentiable HPs & Differential    & optimal storage of discarded entropy             & CLS: MNIST + Omniglot \\
      & \cite{li2017hyperband} 2016.03        & hundreds of HPs                & Random (Bandit) & adaptive resource allocation                     & Diverse tasks \\
      & \cite{loshchilov2016cma} 2016.04      & tens of of HPs                 & CMA-ES~\cite{hansen2001completely} & limited time budget; parallel & CLS: MNIST   \\
      & \cite{falkner2018bohb} 2018.07        & tens of of HPs                 & BayesOpt        & adaptive resource control; parallel              & Diverse tasks \\
      & \cite{houthooft2018evolved} 2018.02   & RL loss                        & Evolution       & truncated trajectory; parallel                   & Physics: MuJoCo \\
      & \cite{lorraine2020optimizing} 2019.11 & millions of differentiable HPs & Differential    & Neumann series                                   & Diverse problems \\
      & \cite{dong2021autohas} 2020.06        & MBS + tens of HPs              & REINFORCE       & weight sharing                                   & CLS: six datasets  \\
      & \cite{baik2020meta} 2020.10           & LR + weight decay (Decay)      & Differential    & truncated trajectory                             & Few-shot CLS \\
\midrule
\multirow{8}{*}{\rotatebox[origin=c]{90}{Auto-Deployment}}
    %   & \cite{mao2016resource} 2016.11 & Resource management & REINFORCE &  & \\
      & \cite{mirhoseini2017device} 2017.06 & device placement                            & REINFORCE    & distributed training                      & CLS + translation \\
      & \cite{reagen2017case} 2017.07       & CMOS-based space + Arch. + HP                & BayesOpt     & N/A                                       & CLS: MNIST \\
      & \cite{nardi2019practical} 2018.10   & FPGA space + Arch. + HP                      & BayesOpt     & N/A                                       & N/A \\
    %   & \cite{kwon2018co} 2018.04 & SOC space + Arc.       &     & & image classification \\
      & \cite{parsa2019pabo} 2019.06        & PUMA space~\cite{ankit2019puma} + Arch. + HP & BayesOpt     & N/A                                       & CLS: Flower17/CIFAR \\
      & \cite{jiang2020hardware} 2019.07    & FPGA space + MBS                            & PPO          & fewer epochs; multi-level exploration     & CLS: CIFAR/ImageNet \\
      & \cite{choi2021dance} 2019.06        & Eyeriss space~\cite{chen2016eyeriss} + MBS  & Differential & weight sharing                            & CLS: CIFAR/ImageNet \\
      & \cite{yang2020co} 2020.02           & ASIC space + Arch.                           & REINFORCE    &  N/A                                      & CLS: three datasets \\
      & \cite{zhou2021rethinking} 2021.02   & edge accelerator space + MBS                & PPO          & weight sharing; neural predictor          & CLS: ImageNet + SEG \\
\midrule
\multirow{11}{*}{\rotatebox[origin=c]{90}{Auto-Adaptation}}
      & \cite{sutton1992adapting} 1992.07     & learning rate                    & Differential  & N/A                    & Synthetic data  \\
      & \cite{hochreiter2001learning} 2001.09 & learning algorithm               & Differential  & N/A                    & Synthetic data \\
      & \cite{white2016greedy} 2016.07        & trace hyperparameter             & Differential  & greedy strategy; approximation & Synthetic: Ringworld \\
      & \cite{wang2017learning} 2016.11       & RL algorithm                     & RL            & limit maximum trials   & Markov decision tasks \\
      & \cite{finn2017model} 2017.03          & initialization                   & Differential  & truncated trajectory   & Few-shot CLS \\
      & \cite{jaderberg2017population} 2017.11 & HPs                             & Evolution     & parallelization        & Game: Atari + StarCraft-{\uppercase\expandafter{\romannumeral2}}  \\
      & \cite{xu2018meta} 2018.05             & HPs in return function           & Differential  & gradient approximation & Game: Atari  \\
      & \cite{veeriah2019discovery} 2019.09   & auxiliary task as questions      & Differential  & truncated trajectory   & Synthetic + Game: Atari  \\
      & \cite{du2019sequential} 2019.06       & initialization + LR/Decay + stop & REINFORCE     & limit maximum steps    & Recommendation \\
      & \cite{kirsch2020improving} 2019.10    & RL loss scalar                   & Differential  & truncated trajectory; parallelization   & Game + Physics  \\
      & \cite{xu2020meta} 2020.07             & RL target scalar                 & Differential  & truncated trajectory; single agent      & Game: Atari \\
    %   & \cite{liu2021return} 2021.02          &    &    &  & RL \\
\bottomrule
\end{tabular}
\label{table:autodl-dissect}
\end{center}
\textit{The algorithms are sorted chronologically.
To save space, we use ``RNS'', ``MBS'', ``Arch.'' and ``HP'' to indicate ``reduced NASNet space'', ``MBConv-based space'', ``architecture search space'', and ``hyperparameters'', respectively.
``CLS'', ``DET'', and ``SEG'' indicate ``classification'', ``detection'', and ``segmentation'', respectively.
Most Auto-Adaptation methods could be categorized into HPO.
}
\end{table*}

==> tables/table-paradigms.tex <==
\begin{table*}[!htb]
\begin{center}
% \setlength{\tabcolsep}{1pt}
\caption{
The most common approaches underlying adaptive strategies for AutoDL.
}
\begin{tabular}{llll}
\toprule
Maintenance Approach & \makecell[l]{Domain\\ Constraints\\$(\gS_1\rightarrow\gS_2)$} & \makecell[l]{Data Availability\\for Maintenance\\$(\gS_2)$} 
& Notes
\\
\midrule
Continuous Learning    & None                                                               & Any 
& \makecell[l]{Constantly processes a data stream.\\Can combine with other approaches.}
\\
Domain Adaptation      & $\mathbb{Y}_1=\mathbb{Y}_2$                                        & $x$: \cmark, $y$: \xmark \\
Domain Generalization  & $\mathbb{Y}_1=\mathbb{Y}_2$                                        & $x$: \xmark, $y$: \xmark 
& Often generalizes more than one domain.
\\
Few-shot Learning      & $\mathbb{Y}_1\neq\mathbb{Y}_2$                                     & $x$: \cmark, $y$: \cmark 
& Prioritizes minimal sampling of $\gS_2$.
\\
Zero-shot Learning     & $\mathbb{Y}_1\neq\mathbb{Y}_2$                                     & $x$: \xmark, $y$: \cmark \\
\bottomrule
\end{tabular}
\label{table:paradigms}
\end{center}
\textit{
    Sample $\gS_i$ represents a domain indexed by $i$, where $\mathbb{Y}_i$ is its corresponding output/label space. The inputs and output labels within sample data are represented by $x$ and $y$, respectively. Domain adaptation/generalization is well-suited for statistical shifts and concept drifts, given a fixed task, while low-shot learning quickly adapts to new classes, a consequence of task redefinition. Note that there are proposed variants to these approaches, e.g., differing degrees of label-based supervision from $\gS_2$.
}
\end{table*}


% \begin{table*}[t!]
% \begin{center}
% \setlength{\tabcolsep}{1pt}
% \caption{
% The most common approaches underlying adaptive strategies for AutoDL.
% }
%     \begin{tabular}{l l l l l l}
%     \toprule
% Principles             & \makecell[l]{Training\\Domain}               & \makecell[l]{Test\\Domain} & \makecell[l]{Access of data\\$(x,y){\sim}(\gX,\gY)$ in $\gS$}            & \makecell[l]{Data Summary}  & Explanation \\
%     \midrule
% % The i.i.d. Assumption & $\gS$                                        & $\gS$                      & $x,y$: \cmark
% %                       & $\gX$ does not change  & The estimated distribution differs from $\gX$. \\
% Domain Adaptation     & $\gS^\textrm{source}, \gS^{\textrm{target}}$ & $\gS^{\textrm{target}}$    & $x^{\textrm{target}}$: \cmark, $y^{\textrm{target}}$: \xmark
%                       &  $\mathbb{Y}^\textrm{source}{=}\mathbb{Y}^\textrm{target}$ & Access to unlabeled data of the target domain \\
% Domain Generalization & $\gS^{1}, ..., \gS^{n}$                      & $\gS^{n+1}$                & $(x,y)^{n+1}$: \xmark
%                       & $\mathbb{Y}^{i}{=}\mathbb{Y}^{j}, s.t.~1{\leq}i{\neq}j{\leq}{n+1}$
%                       & Generalize to an unseen target domain $\gS^{n+1}$ \\
% % Multi-task Learning   & $\gS^{1}, ..., \gS^{n}$                      & $\gS^{1}, ..., \gS^{n}$    & $(x,y)^{1{\leq}{i}{\leq}{n}}$: \cmark
% %                       & $\mathbb{Y}^{i}{\neq}\mathbb{Y}^{j}, s.t.~1{\leq}i{\neq}j{\leq}{n}$
% %                       & \\
% Few-shot Learning     & $\gS^{1}, ..., \gS^{n}$                      & $\gS^{n+1}$                & $(x,y)^{n+1}$: \cmark
%                       & $\mathbb{Y}^{i}{\neq}\mathbb{Y}^{j}, s.t.~1{\leq}i{\neq}j{\leq}{n+1}$
%                       & Adapt to new domain with unseen classes.     \\
% Zero-shot Learning    & $\gS^\textrm{seen}$                          & $\gS^\textrm{unseen}$      & \makecell[l]{$x^\textrm{unseen}$: \xmark\\$y^\textrm{unseen}$: \hmark}
%                       & $\mathbb{Y}^\textrm{seen}{\neq}\mathbb{Y}^\textrm{unseen}$
%                       & \makecell[l]{Generalize to data of unseen classes with\\class-level attribute being available.} \\
% Continuous Learning    & $\gS^{1}, ..., \gS^{t}$                      & $\gS^{1{\leq}i{\leq}t}, \gS^{t+1}$                & $(x,y)^{t+1}$: \cmark
%                       & $\mathbb{Y}^{i}{\neq}\mathbb{Y}^{j}, s.t.~1{\leq}i{\neq}j{\leq}{t+1}$
%                       & \makecell[l]{$S^{t}$ arrives sequentially.\\Label space $\mathbb{Y}$ changes over time.} \\
% % Concept Drift         & $\gS^{1}, ..., \gS^{t}$                      & $\gS^{t+1}$                & $(x,y)^{t+1}$: \cmark
% %                       & \makecell[l]{$\Pr(y^{i} | x^{i}){\neq}\Pr(y^{j} | x^{j})$\\$\mathbb{Y}^{i}{=}\mathbb{Y}^{j}, ~s.t.~1{\leq}i{\neq}j{\leq}{t+1}$}
% %                       & \makecell[l]{$S^{t}$ arrives sequentially. The oracle\\mapping $\Pr(y | x)$ changes over time.} \\
%     \bottomrule
%     \end{tabular}
%     \label{table:paradigms}
%     \end{center}
% \textit{
% $\gS$ indicates the domain.
% $\gX$ and $\gY$ indicate the distribution of sample and label in the domain $\gS$, respectively.
% $x$ and $y$ refer to a sample and its label sampled from the distribution $\gX$ and $\gY$.
% $\mathbb{Y}$ indicates the label space.
% In domain adaptation, there are two (source and target) domains.
% In domain generalization, the model is trained on $n$ domains and is expected to generalize on a different ($n+1$-th) domain.
% In few-shot learning, the model needs to quickly solve a new task (viewed as a domain in this table) with a few data available.
% In zero-shot learning, the model is trained on data with seen classes and is expected to generalize to unseen classes.
% For continual learning and concept drift, the domain, as well as the corresponding data, comes sequentially over time, from $1$-th to $t$-th domain.
% }
% \end{table*}

==> tables/table-questionnaire.tex <==


\newcommand{\answerYes}[1][]{\textcolor{blue}{[Yes] #1}}
\newcommand{\answerNo}[1][]{\textcolor{orange}{[No] #1}}
\newcommand{\answerNA}[1][]{\textcolor{gray}{[N/A] #1}}
\newcommand{\LACK}[1]{{\textcolor{red}{#1}}}
\newcommand{\EX}[1]{{\textcolor{purple}{#1}}}
\newcommand{\answerTODO}[1][]{\textcolor{red}{\bf [TODO]}}
\newcommand{\didmark}{\ding{51}}
\newcommand{\notmark}{\ding{55}}

  
\begin{table*}[!htp]
\begin{center}
\setlength{\tabcolsep}{3pt}
\caption{
An example self-assessment questionnaire for AutoDL algorithms.
}
% \begin{tabular}{ l | l | l }
\begin{tabularx}{\linewidth}{ p{0.1\linewidth} | p{0.4\linewidth} |
% p{0.22\linewidth} | 
X }
\toprule
              & Question 
            %   & Response 
              & Example response for NASNet~\cite{zoph2018learning} \\
\midrule
\multirow{6}{*}{Novelty}
       & Is there significant innovation in this work?        
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & Yes; the first cell-based search space in NAS. \\
       & Is this work completely distinct from existing research in Automated Data Engineering?        
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & Yes; within reasonable scope. \\
       & Is this work completely distinct from existing research in NAS?        
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & No, but without issue; reuses the search method in \cite{zoph2017NAS}. \\
       & Is this work completely distinct from existing research in HPO?       
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & No, but without issue; the search method has been studied in HPO. \\
       & Is this work completely distinct from existing research in Automated Deployment?                  
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & Yes; within reasonable scope. \\
       & Is this work completely distinct from existing research in Automated Maintenance?                  
    %   & \underline{\answerYes or \answerNo}, \EX{\underline{...}} 
       & Yes; within reasonable scope. \\
\midrule
\multirow{6}{*}{{\makecell[l]{Solution\\Quality}}}
      & Does the contribution of this AutoDL method to model accuracy (or similar metric) significantly improve upon equivalent SoTA approaches? 
    %   & \EX{\underline{...}} 
      & No, but without issue; the largest NASNet model (of the time) achieves 82.7\% top-1 accuracy on ImageNet, which is similar to previous SoTA model but with 40\% reduction in FLOPs. \\
      & Is the reported contribution to accuracy (or similar metric) fairly representative? 
    %   & \EX{Reported on \underline{xxx} datasets}                 
      & Yes, decently; reported for CIFAR-10, ImageNet, COCO. \\
    %   & How is the reported accuracy fairly compared with the previous SoTA performance? & \EX{\underline{...}} & As of July 2017, the largest NASNet model can achieve 82.7\% top-1 accuracy on ImageNet, which is similar to previous SoTA model but reduced about 40\% FLOPs. \\
\midrule
\multirow{5}{*}{Efficiency}
      & Does this AutoDL method converge with significant speed?                 
    %   & \EX{\underline{x} epochs, \underline{y} GPU hours}            
      & Yes; 2000 NVidia P100-hours to complete NAS on CIFAR-10. \\
      & Does the contribution of this AutoDL method to model efficiency (i.e., minimization of computational-resource usage) significantly improve upon equivalent SoTA approaches?             
    %   & \EX{FLOPs: \underline{x}, \#Parameters: \underline{y}}        
      & Yes; this NAS method can produce a model with 3.3 million parameters that achieves 3.41\% error on CIFAR-10, \LACK{but latency is not evaluated.} \\
      & Are the theoretical/practical efficiencies fairly analyzed? 
    %   & \underline{\answerYes or \answerNo}; \EX{\underline{x\% absolute}} \EX{\underline{and y\% relative gain}} 
      & Yes, mostly; the number of model parameters and FLOPs are analyzed, \LACK{although there is no comment on practical speed}. \\
\midrule
\multirow{5}{*}{Stability}
       & Do repeated runs of this AutoDL method produce results (e.g., in terms of accuracy metric) with minimal variance? 
    %   & \EX{\underline{over all $\leq x_{1}$,}}; \EX{\underline{specifically}} \EX{\underline{$\leq x_{2}$}} \EX{\underline{on $d_1$ dataset, etc.}} 
       & Unknown; \LACK{analysis does not exist.} \\
       & Do repeated runs of this AutoDL method impact model structure (if applicable) in the same way?       
    %   & \underline{\answerYes or \answerNo} 
       & Unknown; \LACK{although NAS methods intrinsically influence model structure by virtue of construction, analysis does not exist.} \\
       & Is the AutoDL method stable (i.e., not sensitive) for certain values of AutoDL-method parameters?        
    %   & \underline{\answerYes or \answerNo} 
       & Yes, with minimal analysis; brief mention that a learning rate of 3.5e-4 is relatively stable. \\
\midrule
\multirow{4}{*}{{\makecell[l]{Interpret-\\ability}}}
       & Is this AutoDL method explainable in how it impacts the target model?                            
    %   & \EX{\underline{...}} 
       & Unknown; \LACK{analysis does not exist.} \\
       & Are the results produced by the target model (after the AutoDL method takes effect) explainable?               
    %   & \EX{\underline{...}} 
       & Unknown; \LACK{analysis does not exist.} \\
\midrule
\multirow{10}{*}{\makecell[l]{Reproduc-\\ibility}}
      & Is all relevant experimental code involving this AutoDL method publicly available?            
    %   & \underline{\answerYes or \answerNo} 
      & No.  \\
      & Are all relevant experimental values for AutoDL-method parameters reported in the paper/code?       
    %   & \underline{\answerYes or \answerNo} 
      & Yes, mostly. \\
      & Is all relevant experimental code involving the models resulting from this AutoDL method publicly available?      
    %   & \underline{\answerYes or \answerNo} 
      & Yes. \\
      & Are all relevant experimental values for resulting models (e.g., hyperparameters) reported in the paper/code?  
    %   & \underline{\answerYes or \answerNo} 
      & Yes. \\
      & Is miscellaneous experimental information (e.g., random seed, hardware, or platform) reported?     
    %   & \underline{\answerYes or \answerNo} 
      & Yes, decently; hardware and platform are mentioned. \\
\midrule
\multirow{9}{*}{\makecell[l]{Engineering\\Quality}}
      & Is this AutoDL method implemented for public use (e.g., off-the-shelf scripts)? 
    %   & \EX{\underline{x/y/z} for search/train/test}     
      & Yes, but minimally; there is one script.         \\
      & Is the implementation code commented?               
    %   & \EX{\underline{$\frac{x}{y}$} key classes/funcs} 
      & Yes, partially. \\
      & Is the implementation code tested?             
    %   & \EX{\underline{x\%} via Codecov}                 
      & Yes, mostly; \LACK{however, there is a lack of detailed test reports.} \\
      & Is the implementation code documented?   
    %   & \underline{\answerYes or \answerNo}              
      & Yes; for model training/evaluation. \\
      & Is the implementation code modular, reusable, and extendable?             
    %   &  \EX{\underline{.....}}                          
      & Yes; different config files can instantiate different versions of NASNet. \\
\midrule
\multirow{7}{*}{Scalability}
       & Are the theoretical/practical computational costs of this AutoDL method analyzed?           
    %   & \underline{\answerYes or \answerNo} 
       & Yes, partially; empirical costs are analyzed, \LACK{theoretical costs are not}. \\
       & Is it feasible to scale up to large-scale datasets? 
    %   & \underline{\answerYes or \answerNo} 
       & No, but issue considered; sub-networks (i.e., cells) discovered for small-scale datasets can be transferred to large-scale datasets. \\
       & Is it feasible to scale up to large-scale models?         
    %   & \underline{\answerYes or \answerNo} 
       & Unknown; \LACK{analysis does not exist.} \\
       & Is it feasible to scale up to large-scale search spaces?   
    %   & \underline{\answerYes or \answerNo} 
       & Unknown; \LACK{analysis does not exist.} \\
\midrule
\multirow{5}{*}{\makecell[l]{Generaliz-\\ability}}
       & Can this AutoDL method generalize well to unseen datasets?       
    %   & \underline{\answerYes or \answerNo}, \EX{what datasets?} 
       & Yes; from CIFAR to ImageNet and COCO. \\
       & Can this AutoDL method generalize well to different target models? 
    %   & \underline{\answerYes or \answerNo}, \EX{what models?} 
       & Yes; can generalize to other macro structures. \\
       & Can this AutoDL method generalize well to different kinds of search spaces?        
    %   & \EX{\underline{...}} 
       & No, but without issue; the proposed NASNet search space is intrinsic to the NAS algorithm. \\
\midrule
\multirow{5}{*}{\makecell[l]{Eco-friend-\\liness}}
       & Is the energy consumption minimal for this AutoDL method?
    %   & \EX{\underline{...}} 
       & Unknown; \LACK{analysis does not exist.}\\
       & Is the energy consumption minimal for the target model when actively employed?          
    %   & \EX{\underline{...}} 
       & Unknown; \LACK{analysis does not exist.}\\
       & Is the potential environmental impact of this AutoDL method (e.g., converted to carbon emissions) minimized?                 
    %   & \EX{\underline{N/A}} 
       & Unknown; \LACK{analysis does not exist.}\\
\bottomrule
\end{tabularx}
\label{table:autodl-questionnaire}
\end{center}
\textit{
AutoDL algorithms need to be evaluated from these ten aspects.
This questionnaire is the minimal coverage and should definitely be upgraded as time goes.
We use a seminal NAS work, NASNet~\cite{zoph2018learning}, as an example to show the usage of this questionnaire.
All comparisons are made against the available literature of the time, i.e., July 2017.
% Abbreviations are: ``N.A.'' for ``not applicable''.
}
\end{table*}


==> tables/table-scenarios.tex <==
\begin{table}[!htb]
\begin{center}
\caption{
Scenarios in a dynamic data environment.
}
\begin{tabular}{ll}
\toprule
Scenario             & \makecell[l]{Changes\\ $(\gS_1\rightarrow\gS_2)$} \\ \midrule
The i.i.d. Assumption & None                                \\
Covariate Shift       & $P(x)$                              \\
Prior Shift           & $P(y)$                              \\
Concept Drift         & $P(y|x)$                            \\
Task Redefinition     & $\mathbb{X}$ and/or $\mathbb{Y}$    \\
\bottomrule                  
\end{tabular}
\label{table:dynamics}
\end{center}\textit{
    Set $\gS_i$ is defined here as a collection of data that samples an input-output distribution of interest to a DL model, i.e., a domain indexed by $i$. Input $x$ and output label $y$ belong to input and output spaces $\mathbb{X}$ and $\mathbb{Y}$, respectively, while $P$ denotes a probability with respect to sampling representation.
    }
\end{table}
